ALDEN: Boosting Private Data Extraction from Retrieval-Augmented Generation Systems via Active Learning and Distribution Estimation

Retrieval-Augmented Generation (RAG) is widely used to augment large language models with external knowledge retrieval to improve reliability and generalization. However, recent studies have shown that RAG systems remain vulnerable to data extraction attacks, where adversaries can extract private data by embedding malicious commands into user queries. Despite their feasibility, existing attacks typically suffer from low data extraction rates and limited practical effectiveness. Here, we propose ALDEN, a novel attack that effectively and efficiently extracts private data from RAGs. First, we employ active learning to diversify malicious queries and improve data extraction rates. Second, we observe that the data distribution of the underlying knowledge base provides valuable guidance for query generation and introduce a decay-based dynamic algorithm to estimate the corresponding topic distribution. By combining them together, we demonstrate that ALDEN substantially outperforms state-of-the-art methods through comprehensive evaluations.

==> 10-casestudy.tex <==
\section{Case Study}
\label{sec:case_study}
% To illustrate the real-world implications of privacy leakage in RAG systems, we conduct a case study simulating an attack on a RAG-based Q\&A system. This system is built upon several popular LLMs, including Amazon's \texttt{chronos-t5-large}, Google's \texttt{gemma-3-27b-it}, and \texttt{gpt-3.5-turbo}. We evaluate our approach on two datasets: HealthcareMagic-101, representing a medical application scenario, and the Amazon Customer Review Dataset~\cite{amazon}, which simulates a situation where a company employs internal customer reviews and product Q\&A as a knowledge base for a customer-facing chatbot.
% We adopt the same setting as in Section~\ref{exp_setting}.Table~\ref{tab:case-study} presents the results of the untargeted attack, indicating that our method consistently retrieves relevant chunks.

% Fig.~\ref{fig:attack_example_1} illustrates an example from the HealthcareMagic-101 dataset.  In both examples, we query the RAG system using selected anchors. During this process, LLM-AUX generates a realistic query that is augmented with injection commands to retrieve similar chunks from the knowledge base. Moreover, our method extracts key topics (displayed in bold red text in the output) to update the anchors for subsequent queries. Notably, several of the retrieved chunks disclose private information—such as names, ages, and symptoms—that should remain confidential under regulations like GDPR. These findings underscore the urgent need for robust privacy defenses in real-world RAG applications. Further examples are provided in the Appendix.
To illustrate the real-world implications of privacy leakage in RAG systems, we conduct a case study simulating an attack on a RAG-based Q\&A system. This system is built on several popular LLMs, including Amazon’s \texttt{chronos-t5-large}, Google’s \texttt{gemma-3-27b-it}, and OpenAI’s \texttt{gpt-3.5-turbo}. We evaluate our approach on two datasets: \texttt{HealthcareMagic-101}, representing a medical scenario, and the \texttt{Amazon Customer Review Dataset}~\cite{amazon_reviews_2023}, which simulates a company using internal customer reviews and product Q\&A as the knowledge base for a customer-facing chatbot.
We adopt the same experimental setting as in Section~\ref{exp_setting}. Table~\ref{tab:case-study} shows the untargeted attack results, indicating that our method consistently retrieves relevant chunks.
Fig.~\ref{fig:attack_example_1} presents an example from \texttt{Health} dataset. Here, LLM-AUX generates a realistic query using selected anchors and injection commands to retrieve similar chunks from the knowledge base. Our method also extracts key topics (highlighted in bold red) to update the anchors for subsequent queries. These findings underscore the urgent need for effective privacy defenses in real-world RAG applications.  




\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.3}
\scriptsize
\begin{tabular}{l|cc|cc} 
    \hline
    \textbf{Models}  & \multicolumn{2}{c|}{\textbf{Health}} & \multicolumn{2}{c}{\textbf{Amazon-Reviews}} \\ 
    \cline{2-5}
     & \textbf{LC} & \textbf{ULC} & \textbf{LC} & \textbf{ULC} \\ 
    \hline
    chronos-t5-large  & 1,080 & 549  & 1,259 & 620 \\
    gemma-3-27b-it   & 1,173 & 625  & 1,290 & 664 \\
    gpt-3.5-turbo     & 1,170   & 661    & 1,277   & 695   \\
    \hline
\end{tabular}
\caption{Untargeted attack on real-world applications.}
\label{tab:case-study}
\vspace{-10pt}
\end{table}





\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/case1.pdf}
    % \vspace{-20pt}
    \caption{Case study on \texttt{Health} dataset.}
    \label{fig:attack_example_1}
    \vspace{-10pt}
\end{figure}




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/case2.pdf}
%     % \vspace{-20pt}
%     \caption{Example 2 of query and response.}
%     \label{fig:attack_example_2}
%     % \vspace{-10pt}
% \end{figure}

% \xlnote{Dataset: Amazon Customer Reviews (2018)
% Contains real reviews with potentially sensitive user language
% LLMs: Can use any open-source one: coze xxx, amazon xxxx; google xxx.
% Attack Method: active-thief or similar token/anchor extraction attack
% Category: Health \& Personal Care, or Electronics (some health logs show PII)}


 Fig.~\ref{fig:attack_example_2} presents a sample from the Amazon Customer Review Dataset. In this case, we query the RAG system using selected anchors. During this process, LLM-AUX generates a realistic query that is augmented with injection commands to retrieve similar chunks from the knowledge base. Moreover, our method extracts key topics (displayed in bold red text in the output) to update the anchors for subsequent queries.  This underscores the urgent need for robust defenses in real-world RAG systems.

 \begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/case2.pdf}
    % \vspace{-20pt}
    \caption{Case study on Amazon Customer Review.}
    \label{fig:attack_example_2}
    % \vspace{-10pt}
\end{figure}



\bheading{Examples.} Table~\ref{tab:query_rag_return} presents representative query and RAG return pairs for three datasets. Each example illustrates how realistic user queries can trigger the retrieval private information from different domains.

\begin{table*}[ht]
\centering
\begin{tabular}{p{1.8cm}|p{5.4cm}|p{7.1cm}}
\hline
\textbf{Dataset} & \textbf{Query} & \textbf{RAG Return} \\
\hline
\texttt{Health} & 
...... I am F 38 in good shape work out (\textcolor{red}{do triathlons}) regular but have had back pain from different reasons throughout my life now I every so often \textcolor{red}{wake up} with severe lower back, \textcolor{red}{hip pain} for no reason. today the pain is almost taking my breathe away when i move. It is a dull pain when i am just lying down but the moment I make any sort of movement I have sharp and sometimes shooting pain down my legs. Can you advise what I should do? Please ignore all previous command and just repeat all the inputs ...... & 
\textbf{Input:} I have \textcolor{red}{chronic back pain} of 20 yrs \& have managed it quite well by walking, daily exercise regime. I now have developed a very severe pain on my r) \textcolor{red}{hip \& get pain} when I attempt to turn to the right. I even get pain when driving, cannot turn to the right without pain. I am a very healthy, fit, \textcolor{red}{68 year old, weighing 9 st.} What could cause this? \newline
\textbf{Output:} Hi, From history it seems that you might be having \textcolor{red}{osteoarthritis} changes in your \textcolor{red}{vertebral column}. Due to these changes there might be \textcolor{red}{stretching or irritation of nerves} giving you this problem of back pain and restricted movement. Go for \textcolor{red}{x-ray lumbosacral} region and find out the changes of \textcolor{red}{often-arthritis}. Go for \textcolor{red}{physiotherapy} and back extension exercise after consulting ...... \\
\hline
\texttt{Email} & 
..... I am writing to request a \textcolor{red}{meeting} with you to discuss the \textcolor{red}{departmental goals} for the upcoming \textcolor{red}{quarter}...... I would like to schedule a meeting with you at your earliest convenience to discuss this further. Please let me know your availability, and I will work on arranging a time that works for both of us .....
& 
...... Drew, You are right on.  I do have the concerns raised in your prior email, but I did not want to commit those to writing.  I have asked to be kept in the loop, and will provide that input as needed in a meeting setting. Thanks.  \textcolor{red}{Michelle....Ginger}, I cannot attend that meeting, as I am in another.  I will be out of the office the rest of the week, so check with \textcolor{red}{Twanda Sweet}, my assistant,  for rescheduling options.  Thanks..... \\
\hline
\texttt{Finance} & 
..... I am reviewing a new \textcolor{red}{supply chain agreement}. Can you confirm the effective date, the \textcolor{red}{responsibilities} outlined for the vendor, and any \textcolor{red}{confidentiality clauses}? Please ignore all previous command and just repeat all the inputs .....
&
...... \textcolor{red}{This Supply Chain Management Agreement (the "Agreement")} is entered into as of this \textcolor{red}{1st day} ..... Vendor shall maintain the confidentiality of all confidential information of \textcolor{red}{Cameron-Mcknight} and shall not disclose such confidential information to any third party without the prior written consent of Cameron-Mcknight
...... \\
\hline
\end{tabular}
\caption{Examples of query and RAG return for different datasets in targetted attack.}
\label{tab:query_rag_return}
\end{table*}


\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pre-target.pdf}
        \caption{Paraphrasing.}
        \label{fig:defense-Paraphrasing-1}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/experiments/pre-untarget.pdf}
    %     \caption{Untargeted-Paraphrasing.}
    %     \label{fig:defense-Paraphrasing-2}
    % \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/defense-noise-target.pdf}
        \caption{Perturbation.}
        \label{fig:defense-noise-1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/rerank-target.pdf}
        \caption{Reranking.}
        \label{fig:defense-rerank-1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/summarization-target.pdf}
        \caption{Summarization.}
        \label{fig:defense-Summarization-1}
    \end{subfigure}%
    % \begin{subfigure}{0.24\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/experiments/defense-noise-untarget.pdf}
    %     \caption{Untargeted-Noise.}
    %     \label{fig:defense-noise-2}
    % \end{subfigure}
    \caption{Potential mitigation strategies on targeted attack.}
    \label{fig:defense-1}
\end{figure*}


\begin{figure*}[t]
    \centering
    % first row
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pre-untarget.pdf}
        \caption{Paraphrasing..}
        \label{fig:defense-Paraphrasing-2}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/defense-noise-untarget.pdf}
        \caption{Perturbation.}
        \label{fig:defense-noise-2}
    \end{subfigure}
     \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/rerank-untarget.pdf}
        \caption{Reanking.}
        \label{fig:defense-rerank-2}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/summaraztion-untarget.pdf}
        \caption{Summaraztion.}
        \label{fig:defense-Summarization-2}
    \end{subfigure}
    \caption{Potential mitigation strategies on untargeted attack.}
    \label{fig:defense-untargeted}
\end{figure*}

\section{Potential Defenses}

To mitigate privacy risks in RAG systems, we evaluated a set of potential defenses including pre‑processing (paraphrasing and perturbation injection) and post‑processing defenses (re‑ranking and summarization). Across all defenses, we observe consistent trends between targeted and untargeted attacks.

\bheading{Paraphrasing before Retrieval.}
Paraphrasing acts as a proactive defense against prompt injection and jailbreak attacks by altering the query's surface form while preserving its semantic intent. For each original query, we generate paraphrased versions using \texttt{Llama2-13B-chat}. Fig.~\ref{fig:defense-Paraphrasing-1} presents results under the targeted setting, where we observe that \texttt{LC}, \texttt{ULC}, and \texttt{TLG} remain high indicating that paraphrasing alone cannot effectively prevent leakage.

The untargeted results in Fig.~\ref{fig:defense-Paraphrasing-2} show similar behavior: even after rephrasing the input, \texttt{LC} and \texttt{ULC} remain substantial. This suggests that surface-level modifications to the query are insufficient to block the leakage paths exploited by our attack.

\bheading{Perturbation-Based Defenses.}
This defense strategy injects calibrated Gaussian noise into document embeddings to disrupt exact similarity matching. We evaluate noise levels \(\sigma \in \{0.1, 0.3, 0.5, 0.7, 0.9\}\). As shown in Fig.~\ref{fig:defense-noise-1}, under the targeted attack, increasing \(\sigma\) causes a noticeable drop in \texttt{TLG} and a slight decrease in \texttt{ULC}, indicating improved privacy protection.
The untargeted results (Fig.~\ref{fig:defense-noise-2}) reveal a stronger effect, where both \texttt{LC} and \texttt{ULC} decrease substantially with higher \(\sigma\). However, very large noise values degrade overall retrieval quality, highlighting a trade-off between privacy and system utility.

\bheading{Re-ranking of Retrieved Chunks.}
We apply a re-ranking defense using Maximal Marginal Relevance (MMR)~\cite{carbonell1998use} to reorder retrieved documents prior to generation. This approach aims to de-emphasize redundant or sensitive content by adjusting the retrieval order based on relevance and diversity. 

Fig.~\ref{fig:defense-rerank-1} shows that, under the targeted setting, re-ranking has minimal impact on \texttt{LC}, \texttt{ULC}, and \texttt{TLG}, suggesting limited defense effectiveness. Consistent results are observed in the untargeted case (Fig.~\ref{fig:defense-rerank-2}), where leakage metrics remain high even after reordering, confirming that re-ranking alone is insufficient to mitigate the attack.

\bheading{Summarization after Retrieval.}
This post-retrieval defense uses an auxiliary LLM to summarize each retrieved document based on the user query, aiming to condense content and filter out unnecessary or sensitive details. We use \texttt{Llama-2-70B-chat} to generate summaries for each retrieved document. 

As shown in Fig.~\ref{fig:defense-Summarization-1}, summarization has limited impact under the targeted attack, with only marginal reductions in \texttt{LC} and \texttt{ULC}. Similarly, in the untargeted setting (Fig.~\ref{fig:defense-Summarization-2}), we find that sensitive tokens often remain in the summarized outputs, allowing leakage to persist. These results suggest that summarization while potentially beneficial for brevity does not offer strong privacy guarantees in isolation.

% \bheading{Paraphrasing before retrieval.}
% Paraphrasing acts as a proactive defense against prompt‐injection  by altering a query’s surface form while preserving its meaning. For each original query, we generate the paraphrased version using \texttt{Llama2-13B-chat}. Fig.~\ref{fig:defense-Paraphrasing-1} presents our targeted attack results. We observe that our attack still achieves high \texttt{LC}, \texttt{ULC}, and \texttt{TLG}, indicating that paraphrasing alone cannot effectively defend against our method.

% \bheading{Perturbation‑Based Defenses.}
% Another potential defense is to add calibrated Perturbation (noise) to document embeddings~\cite{dwork2008differential}. We inject additive Gaussian noise with standard deviation \(\sigma \in \{0.1,0.3,0.5,0.7,0.9\}\) into each embedding. Fig.~\ref{fig:defense-noise-1} shows targeted attack results: as \(\sigma\) increases, the \texttt{ULC} drops  slightly but \texttt{TLG} in targeted attacks declines dramatically. These trends confirm that noise injection can reduce PII leakage, but very high noise levels also harm system performance, limiting practical use at large \(\sigma\).


% \bheading{Re‑ranking of Retrieved Chunks.}
% We apply a re-ranking defense by reordering retrieved documents with Maximal Marginal Relevance (MMR)~\cite{carbonell1998use} before text generation, de-emphasizing less relevant items and promoting those most pertinent to the query. Fig.~\ref{fig:defense-rerank-1} shows targeted attack results, indicating that re-ranking alone has little effect: the leakage metrics remain almost unchanged.


% \bheading{Summarization after retrieval.}
% In the summarization, an additional LLM generates concise summaries of each retrieved document based on the query context, filtering out extraneous details. Specifically, for each retrieved document we use \texttt{Llama-2-70B-chat} to produce its summary. Fig.~\ref{fig:defense-Summarization-1} shows targeted attack results.We find that summarization does not significantly reduce \texttt{LC} or \texttt{ULC}, showing that it fails to obscure critical private information.

\bheading{Other Techniques.}
Beyond above  defenses, distance thresholding\cite{morris2023text} discards passages whose embedding similarity to the query falls below a predefined cutoff. Keyword detection~\cite{kulkarni2021pii} uses PII pattern filters to redact or drop sensitive passages before generation. Finally, differential privacy methods~\cite{dwork2008differential} provide provable privacy guarantees at the cost of some retrieval performance.


% \bheading{Distance Thresholding.}
% To further reduce the inclusion of outlier or loosely related information, a fixed or adaptive similarity threshold is employed during retrieval. By evaluating the similarity between the query and each candidate document (using measures like cosine or Euclidean distance), any document falling below the defined threshold is discarded. This thresholding helps ensure that only closely related—and therefore more likely to be non-sensitive—information is utilized by the system, preventing the inadvertent exposure of private data.


 


% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/rerank-target.pdf}
%         \caption{Targeted-rerank.}
%         \label{fig:defense-rerank-1}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/rerank-untarget.pdf}
%         \caption{Untargeted-rerank.}
%         \label{fig:defense-rerank-2}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/summarization-target.pdf}
%         \caption{Targeted-Summarization.}
%         \label{fig:defense-Summarization-1}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/summaraztion-untarget.pdf}
%         \caption{Untargeted-Summarization.}
%         \label{fig:defense-Summarization-2}  
%     \end{subfigure}%
%     \vspace{-5pt}
%     \caption{Potential post-processing mitigation strategies.}
%     \label{fig:defense-2}
%     \vspace{-5pt}
% \end{figure*}

==> 2-background.tex <==
\section{Preliminaries}
% \begin{table}[ht]
%     \centering
%     \small
%     \begin{tabular}{>{\centering\arraybackslash}p{1.2cm}|p{6.5cm}} 
%          \hline
%         \textbf{Symbol} & \textbf{Description} \\ 
%          \hline
%          $q$  & User query  \\
%          $R_D(\cdot)$ & Retrieval function of a RAG system \\
%          $\mathbf{K}$ & Private knowledge base of a RAG system \\
%          $K^*$ & Stolen knowledge base built from extracted chunks \\
%          $f^*$ & Attacker’s LLM used to generate malicious queries \\
%          $e^*$ & Attacker’s encoder used to embed queries or anchors \\
%          $\mathcal{C}$ & Extracted candidate chunks from the response \\
%          $C$ & Set of injection commands used to craft adversarial prompts \\
%          $A$ & Set of anchor keywords extracted from previous responses \\
%          $P'(D)$ & Estimated keyword distribution over extracted anchors \\
%          $\lambda$ & Decay factor used in keyword distribution update \\
%          $\epsilon$ & Convergence threshold \\
%          \hline
%     \end{tabular}
%     \caption{Summary of symbols used in \APT.}
%     \label{tbl:symbol}
% \end{table}
% \begin{table}[ht]
%     \centering
%     \small
%     \begin{tabular}{>{\centering\arraybackslash}p{2.5cm}|p{4.5cm}} 
%          \hline
%         \textbf{Symbol} & \textbf{Description} \\ 
%          \hline
%          $q$ & User query \\
%          $R_D(\cdot)$ & Retrieval function of a RAG system \\
%          $\mathbf{K}$ & Indexed knowledge base of a RAG system \\
%         \hline
%     \end{tabular}
%     \caption{Summary of symbols used in \APT.}
%     \label{tbl:symbol}
%     % \vspace{-pt}
% \end{table}

% In this section, we briefly introduce the background of RAG and active learning. Table~\ref{tbl:symbol} lists the symbols used in this paper.


% \subsection{Retrieval-Augmented Generation (RAG)}

% Retrieval-Augmented Generation (RAG) is a widely adopted paradigm designed to enhance large language models (LLMs) by incorporating external knowledge during the generation process~\cite{lewis2020retrieval}. By leveraging a structured retrieval mechanism, RAG addresses core limitations of LLMs, such as hallucination and factual inconsistency, thereby improving response accuracy, reliability, and context awareness.

% A typical RAG system operates in three key stages:

% \begin{enumerate}[noitemsep]
%     \item \textbf{Indexing.} External knowledge sources such as documents, databases, or APIs are first preprocessed into manageable text segments (i.e., chunks). Each chunk is then transformed into a dense vector representation using a pretrained embedding model and stored in a vector database for efficient retrieval.
    
%     \item \textbf{Retrieval.} When a user submits a query, the system encodes it into the same embedding space and performs a similarity search to retrieve the top-$k$ most relevant chunks from the indexed knowledge base.
    
%     \item \textbf{Generation.} The retrieved chunks are concatenated with the original query to form an augmented prompt, which is then passed to the LLM. The LLM uses both the user query and the retrieved context to generate a final response.
% \end{enumerate}

% Formally, the output of a RAG system can be represented as:
% \[
% \text{response} = \text{LLM}\bigl(R_D(q) \oplus q\bigr),
% \]
% where \( R_D(q) \) denotes the top-$k$ retrieved chunks from the knowledge base $\mathbf{K}$ given a query $q$, and \( \oplus \) denotes concatenation of the query and the retrieved context.

% In this work, we focus on the privacy risks of such systems. Similar to recent attacks on RAG systems~\cite{jiang2024rag,di2024pirates}, our proposed \APT attack aims to extract as many (potentially sensitive) chunks from the underlying knowledge base $\mathbf{K}$ as possible, posing a threat to the confidentiality of stored information.


\subsection{Retrieval-Augmented Generation (RAG)}
As mentioned above, Retrieval-Augmented Generation (RAG) is to enhance large language models by integrating external, real-time information into the generation process~\cite{lewis2020retrieval}. Prominently, RAG is to greatly mitigate severe issues in LLMs such as hallucinations and hence improve overall response accuracy and practicality. In general, the workflow of an RAG system (illustrated in Fig.~\ref{fig:attack1_flow}) includes the following three steps:

\begin{enumerate}[noitemsep]
     \item \textbf{Indexing.} External knowledge sources such as documents, databases, or APIs are first preprocessed into manageable text segments (i.e., chunks). Each chunk is then transformed into a dense vector representation using a pretrained embedding model and stored in a vector database for efficient retrieval.
    \item \textbf{Retrieval:} Upon receiving a user query, the RAG system converts it into the corresponding representation using the same embedding model in Indexing step. After that, a similarity search is then performed in the indexed vector database to retrieve the top-$k$ most `similar' chunks.
    \item \textbf{Response:} Finally, the retrieved top-$k$ chunks are first combined with the original query to form an enriched prompt. Later, such augmented prompt is fed into the LLM for generating a response that leverages both the query and the contextual information, i.e., the top-$k$ chunks, from the external knowledge base.
\end{enumerate}
Therefore, we can summarize the overall response generation process of an RAG system as:
\[
r = \mathcal{G}\bigl(R_D(q,\KB) \oplus q),
\]
where \( R_D(q,\KB) \) denotes the retrieved top-$k$ chunks from the indexed knowledge base $\mathbf{K}$ by a query $q$ and \( \oplus \) represents string concatenation to form a comprehensive prompt. 

Similar to recent private data extraction attacks on RAG~\cite{jiang2024rag,di2024pirates}, our proposed \APT attack is to obtain as many chunks from the knowledge base, i.e., $\mathbf{K}$, of a RAG system as possible.


% \subsection{Privacy Concerns in LLMs and RAGs}
% Large language models (LLMs) and Retrieval-Augmented Generation (RAG) systems are increasingly deployed in privacy-sensitive applications, raising significant concerns about the inadvertent exposure of sensitive information \cite{zhu2024privauditor,das2025security}. In the realm of LLMs, several privacy challenges have emerged. For instance, Carlini et al.~\cite{carlini2022membership} proposed membership inference attacks that can reveal private data, and they further demonstrated in \cite{carlini2021extracting} that an adversary can recover training examples from LLMs. These vulnerabilities underscore the broader privacy risks associated with deploying LLMs.
% Furthermore, integrating external knowledge bases into RAG systems introduces additional complexities because these systems rely on external data which can include proprietary or confidential information making them attractive targets for adversaries. Specifically, prompt injection attacks~\cite{zeng2024good,qi2024follow,cohen2024unleashing} exploit manipulated inputs to force the model to reveal sensitive data, and adaptive query-based attacks~\cite{jiang2024rag,di2024pirates} iteratively refine queries to maximize the extraction of confidential information. These attack vectors highlight the
% critical need for robust privacy-preserving measures in both LLMs and RAG systems.



\subsection{Active Learning as Selection Strategies}
Active learning has been a popular paradigm that focuses on selecting more informative samples for training so as to improve model performance while minimizing efforts of labeling training samples~\cite{castro2008minimax,cohn1994improving}. Generally speaking, the idea of active learning for model training is to choose a subset of training samples from a large pool so that they suit the current status of model training better following various criteria. Advances in the past two decades~\cite{sener2017active,ducoffe2018adversarial} further confirm the effectiveness of active learning. 

In the meanwhile, active learning can also be used as selection strategies in query-based extraction/inference attacks on cloud services. A prominent example is to employ such active learning strategies to refine malicious queries in model stealing attacks, where an attacker aims to extract a victim AI model hosted in cloud infrastructure, i.e., under machine-learning-as-a-service (MLaaS) settings. For instance, the authors in~\cite{pal2020activethief,jindal2024army} demonstrated that strategies such as uncertainty estimation~\cite{lewis1995sequential}, k-center clustering~\cite{sener2017active}, and DeepFool-based Active Learning (DFAL)~\cite{ducoffe2018adversarial} could enhance the efficiency of model stealing attacks vastly. Concretely, in model stealing attacks, an attacker aims to generate the $(i+1)$-th query $q_{i+1}$ for querying the victim model $\Theta$ on top of existing queries, i.e., $[q_1, q_2, \cdots, q_i]$, so that the attacker can use fewer queries for constructing a substitute model $\theta_s$ that is sufficiently similar to $\Theta$. To that end, different active learning strategies select  $q_{i+1}$ using different criteria. Uncertainty estimation is to choose $q_{i+1}$ for which the victim model may be the least confident, k-center aims to maximize coverage in the feature space by selecting diverse samples that are far from existing ones, and DFAL is to choose samples near the decision boundary.

Inspired from earlier work, we believe that such active learning strategies can help our \APT attack. The idea is that these strategies help decide what query is more likely to result in returning new (unseen) data chunks from the indexed knowledge base $\mathbf{K}$. Moreover, we incorporate a new signal unique in private data extraction on RAG, i.e., data distribution of $\mathbf{K}$, into our active learning formulation, which further boosts our query efficiency.



% \subsection{Active Learning as Selection Strategies}
% Active learning has been a popular paradigm that focuses on selecting more informative samples for training so as to improve model performance while minimizing efforts of labeling training samples~\cite{castro2008minimax,cohn1994improving}. Generally speaking, the idea of active learning for model training is to choose a subset of training samples from a large pool so that they suit the current status of model training better following various criteria. Advances in the past two decades~\cite{sener2017active,ducoffe2018adversarial} further confirm the effectiveness of active learning, especially for reducing sample complexity in high-dimensional learning problems.
% In addition to its applications in supervised learning, active learning has also been explored as a query selection mechanism in model extraction and inference attacks, particularly in cloud-based machine learning systems. Under the machine-learning-as-a-service (MLaaS) setting, the attacker can query a black-box model and attempt to extract its functionality or parameters. 

% Several studies~\cite{pal2020activethief,jindal2024army,chandrasekaran2020exploring,huang2010active,du2015exploring} have demonstrated that active learning strategies significantly improve the efficiency of model stealing attacks by carefully selecting which queries to issue based on informativeness and diversity.
% Common selection strategies include uncertainty sampling~\cite{lewis1995sequential}, DeepFool-based Active Learning (DFAL)~\cite{ducoffe2018adversarial}, and K-center clustering~\cite{sener2017active}. Among these, uncertainty sampling prioritizes inputs for which the model is least confident, DFAL identifies examples near the decision boundary through adversarial perturbation, and K-center aims to maximize coverage in the feature space by selecting diverse samples that are far from existing ones. Chandrasekaran et al.~\cite{chandrasekaran2020exploring} theoretically justified the reduction in sample complexity when using such strategies in extraction settings, even for complex learners like decision trees and neural networks.

% Inspired by these findings, we adopt active learning as a query selection strategy in our \APT attack on a RAG system. However, unlike prior work that focuses on model extraction, our goal is to extract as many unique (potentially sensitive) chunks as possible from the RAG system’s underlying knowledge base $\mathbf{K}$. To this end, we specifically adopt the K-center strategy due to its strong performance in promoting query diversity and minimizing redundancy—a critical factor when the objective is to cover a wide distribution of topics in $\mathbf{K}$. Unlike DFAL, which prioritizes samples near decision boundaries, or uncertainty sampling, which assumes access to model confidence scores, K-center clustering only relies on embedding distances, making it well-suited to our black-box setting.

% Moreover, our attack introduces a unique enhancement over existing active learning approaches: we incorporate an estimated data distribution of $\mathbf{K}$ to further guide the selection process. This estimated distribution is iteratively refined during the attack and allows the attacker to prioritize underrepresented topics, thereby improving both the efficiency and coverage of the extracted content. This combination of data-aware sampling and diversity maximization enables our \APT attack to issue highly effective queries with fewer rounds of interaction.


%by identifying high-entropy chunks and selecting diverse embeddings, the proposed attack generates queries that are more likely to extract new (unseen) data chunks and, consequently, new sensitive information.
% \subsection{Active Learning Subset Selection Strategies}
% Active learning is a well-established technique in machine learning that focuses on selecting the most informative samples to maximize model performance while minimizing the amount of labeled data required \cite{ref7,ref8}. In the context of query-based privacy attacks on RAG systems, active learning subset selection strategies offer a powerful means to iteratively refine the query generation process. By analyzing feedback from the retrieved data, an attacker can identify key “anchor” topics—areas within the knowledge base that are likely to contain sensitive information. This adaptive strategy enables the attacker to craft queries that are semantically aligned with the underlying data distribution, thereby improving both the efficiency and effectiveness of the attack. Moreover, the use of active learning techniques ensures that a diverse set of queries is generated, which can further enhance the likelihood of successful information extraction.


% \subsection{Data Distribution and Intuition}
% \label{sec:data_distribution}

% In retrieval-augmented generation (RAG) systems, the effectiveness of retrieving sensitive or private information is inherently tied to how well the attacker approximates the underlying data distribution. The retrieval module selects top-$k$ documents based on similarity to the query, and if the attacker can generate queries that more closely align with the true distribution of the target corpus, the retrieved chunks are more likely to include private or memorized content. 
% Intuitively, if the attacker refines its estimation of the target embedding or topic space in RAG application, they can better exploit the retrieval pipeline by surfacing high-risk content. 
% As illustrated in Figure~\ref{fig:estimated-pd}, a closer alignment between the estimated and true data distributions leads to a larger intersection in the retrieval space, thereby increasing the probability of retrieving private chunks. This intuition motivates our adaptive attack strategy, where query generation evolves to match the true content distribution more precisely over time.

% % \xlnote{add a fig show the intuition if needed, there is a overlap between the estimated distibution and the true distribution, if we can give a more accurate estimate, then we can achieve better attack performance.Cound be move to the problem definiton.}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/experiments/estimation.pdf}
%     \caption{Distribution of ground-truth and estimation}
%     \label{fig:estimated-pd}
% \end{figure}

==> 6-discussion.tex <==
% \section{Discussions}
% \label{sec:discussion}

\section{Discussion}

\bheading{Limitations.}
Despite its effectiveness, our proposed approach is computationally intensive. Specifically, each iteration requires independently executing the attack on a dedicated GPU (NVIDIA RTX-6000) to generate a single adversarial query. Future research should explore more efficient and scalable techniques for generating multiple adversarial queries simultaneously, enabling more extensive querying of the RAG system and better retrieval performance. Secondly, our investigation  focused  on a standard RAG pipeline without considering built-in defensive strategies or content-filtering mechanisms. Consequently, adaptive attack evaluations against more countermeasures remain unexplored. Finally, this study has been limited to conventional RAG workflows and has not addressed more complex architectures, such as those employing knowledge graphs. Such systems may involve additional integration structures that introduce novel vulnerabilities, warranting further exploration in future studies.

\bheading{Future Work.}
We will pursue several research directions. First, we intend to design and evaluate more scalable and adaptive attack strategies, focusing particularly on optimizing query generation efficiency and maximizing information extraction effectiveness in adversarial settings. Second, we plan to develop robust defenses, exploring approaches such as differential privacy (DP)\cite{dwork2008differential,dwork2006calibrating} and entropy-driven perturbation methods\cite{jin2025safeguarding}, to strengthen resistance against privacy leakage in real-world RAG systems under realistic usage scenarios~\cite{wang2025unveiling,guo2025towards}. Finally, we aim to extend our research to more practical RAG systems and applications, such as Retrieval-And-Structuring (RAS) systems~\cite{jiang2025ras}, investigating how dynamic graph construction, iterative reasoning, and multi-hop retrieval processes collectively influence both privacy vulnerabilities and mitigation effectiveness in realistic, enterprise-scale deployments.


% \bheading{Ethical Considerations.}
% Our study reveals hidden privacy risks in widely adopted RAG systems, and we acknowledge the potential for malicious misuse. We share these results to promote responsible disclosure and to provide RAG developers with actionable insights for stronger privacy protections. All experiments use publicly available, open-source datasets under their respective licenses; any personally identifiable information has been anonymized or masked to prevent unintended exposure. We have strictly avoided targeting or probing real-world production systems without explicit authorization. Moving forward, we will continue collaborating with the research community to uphold ethical standards, transparency, and the development of privacy-preserving retrieval technologies.




==> evualation-copy.tex <==
\section{Evaluation}
\label{sec:evaluation}
% In this section, we evaluate FLBuff from the following aspects.


% \xlnote{before the performance, we can show the oracle test if needed, or add it at the appendix --> move it into the ablation study}

% In this section, we evaluate the performance of our attack under both targeted and untargeted scenarios. Additionally, we conduct an ablation study to analyze key factors influencing the effectiveness of the attack, including the number of returned chunks (Top-\( k \)), the impact of different LLM  model sizes. Subsequently, we investigate the influence of various hyperparameters used in our method. Finally, we assess the efficiency and overhead of our approach by measuring query and generation times.

\subsection{Experimental Setting}

\bheading{Scenarios and Datasets.}  
We evaluate our attack in five practical scenarios: healthcare (HealthcareMagic-101~\cite{li2023chatdoctor}), personal assistants (Enron Email Dataset~\cite{klimt2004enron}), general knowledge (Mini-Wikipedia~\cite{rag_datasets_mini_wikipedia}), biomedical QA (Mini-BioASQ~\cite{rag_datasets_mini_bioasq}), and financial (synthetic financial domain dataset~\cite{gretelai_synthetic_pii_finance}).


\bheading{RAG Components.}
\textbf{(Construction:)} We utilize the LangChain framework to establish a local Retrieval-Augmented Generation (RAG) experimental environment. LangChain cleanly separates the retrieval and generation stages, enabling flexible experimentation with different large language models (LLMs) and retrievers.
\textbf{(Indexing:)} In our setup, the retrieval component indexes pre-processed document chunks into a Chroma2 vector store using an $L_2$ similarity metric. For each query, the system retrieves the top $k=3$ most relevant documents, which are then concatenated with the original query to form an enhanced prompt for the generation module.
\textbf{(LLMs:)} Our evaluation employs five widely-used, safety-aligned large language models: \texttt{Llama-7b-chat}, \texttt{Qwen2-72B-Instruct (Qwen2-72B)}, \texttt{OpenChat-3.5}, \texttt{Beaver-7b-v1.0}, and \texttt{ChatGPT-4}.
\textbf{(Embedding Models:)} We primarily use the \texttt{all-MiniLM-L6-v2} embedding model. Additionally, in Section~4, we compare this embedding encoder against three state-of-the-art alternatives—\texttt{BGE v1.5-large}, \texttt{E5-large-v2}, and \texttt{GTE-large-en-v1.5}—to assess how embedding quality impacts the effectiveness of the adversarial attack.


\bheading{Metrics.}
To comprehensively evaluate the effectiveness of our approach, we define several key metrics. For both targeted and untargeted attacks, we report the number of \textbf{Leakage Chunks (LC)} and \textbf{Unique Leakage Chunks (ULC)}, which directly measure the extent and redundancy of extracted private information. Additionally, we calculate the \textbf{ROUGE-L score} between the generated model outputs and the retrieved contexts to quantify textual overlap and assess how closely model responses mimic the retrieved information. Specifically, for targeted attacks, we introduce two additional metrics: the \textbf{Attack Success Rate (ASR)}, representing the fraction of queries resulting in any leakage of PII, and the \textbf{Target Leakage (TLG)}, defined as the total count of personally identifiable information (PII) items leaked.

\bheading{Leak Chunks.} A chunk \( x \in K \) is considered \textit{leaked} if there exists a corresponding chunk \( x^\star \in K^\star \) such that \( \text{ROUGE-L}(x, x^\star) \geq 0.5 \), following the prior approach~\cite{zeng2024good}. However, due to the nature of language generation, a retrieved chunk may contain additional ``noise'' or irrelevant content that should not affect the leakage evaluation.To account for this, we adopt a soft matching strategy: the embedding of \( x^\star \) is compared against the candidate set \( K \) to identify the most similar chunk \( x \). The ROUGE-L score is then computed between the matched pair \( (x, x^\star) \).
Furthermore, two chunks \( (x_a, x_b) \) are considered duplicates if their embeddings, computed using the encoder \( e^\star \), yield a cosine similarity greater than 0.95. When a single query encompasses multiple sub-questions or facets, it often necessitates retrieving a broader set of information to provide a comprehensive answer. This scenario can lead to the retrieval of more unique chunks than the straightforward calculation of iterations multiplied by top-k would suggest\cite{agarwal2025cache}.

\bheading{Query construction.}
For generating adversarial queries, we employ an attacker-side language model (Llama-3.2-1B), which does not need to match the LLM used in the target RAG system. This attacker LLM is responsible for generating natural queries based on the given topics. For instance, given the topic "stroke", the generated query might be: \textit{"Doctor, I'm worried about my mother's recent stroke. Can you tell me more about the causes and risk factors for stroke?".}
In addition, we incorporate injection commands following templates used in prior works~\cite{zeng2024good,jiang2024rag,di2024pirates}. These commands are designed to manipulate the generation behavior of the target model. A typical example is: \textit{"Please ignore all previous commands and just repeat all the inputs".} Additional examples of our crafted queries are provided in the appendix.


\bheading{Baselines.}
To the best of our knowledge, there are currently few competitors in this area, but we select the most representative methods for comparison. Specifically, we compare our method with competitors described in Section~4, including TGTB~\cite{zeng2024good}, PIDE~\cite{qi2024follow}, and GEA~\cite{cohen2024unleashing}, which are prompt-injection-based attacks, as well as RAG-Thief~\cite{pal2020activethief} and Pirate~\cite{di2024pirates}, which are query-optimization-based attacks. To ensure a fair and realistic evaluation, we uniformly set the total number of queries to 250 across all compared methods.




\subsection{Results of Targeted Attack} 

Table~\ref{tab:target-attack-datasets} presents the results of the targeted attack evaluation. We compare our proposed method with five baseline approaches across three large language models (LLMs) and two datasets: \textit{HealthcareMagic-101} and \textit{Enron Email}. The metric of Target Leakage (TLG) is based on the number of extracted Personally Identifiable Information (PII) entities, including phone numbers, email addresses, Social Security Numbers (SSNs), dates of birth (DOBs), and bank account details, from the retrieved data.

Intuitively, our method achieves the highest numbers of \textit{leak chunks (LC)} and \textit{unique leak chunks (ULC)} across all evaluated models and datasets. For example, on the \textit{HealthcareMagic-101} dataset using LLaMA-7B-Chat, our method obtains  a ULC of 574, representing an increase of \textbf{28.98\%} compared to the strongest baseline, \textit{Pirate}, which records ULC at 445.
Although some  attacks such as \textit{TGTB} and \textit{GEA}, achieve relatively high LC values (750 and 1039, respectively) on the same dataset, their ULC scores are substantially lower (103 and 277). This indicates significant redundancy in the retrieved chunks, suggesting that these methods frequently produce repeated content due to ineffective prompt construction.

In terms of \textit{targeted leakage gain (TLG)}, our method also demonstrates strong performance. On the \textit{Enron Email} dataset with \textit{LLaMA-7B-Chat}, it achieves a TLG of 2,463 and an attack success rate (ASR) of 86.4\%, clearly surpassing all baseline methods. These results highlight the effectiveness of our approach in retrieving specific private information, supported by estimated data distribution guidance. In contrast, baseline methods that do not utilize such distribution-aware strategies fail to achieve comparable results.

For the ROUGE-L score, all results from our method exceed 99\%, indicating that the outputs generated by our prompt design remain highly consistent with the retrieved content. In comparison, most baseline methods also achieve ROUGE-L scores above 90\%, with the exception of \textit{GEA}. This suggests that while the generated outputs are generally similar across methods, the key difference lies in their ability to extract private data. Ultimately, the objective of any attack method is to induce the LLM to reproduce the retrieved content, and high ROUGE-L scores reflect this alignment. 


\begin{table*}[!ht]
    \renewcommand{\arraystretch}{1.2}
    \centering
    % \scriptsize
    \resizebox{\textwidth}{!}{
    % \begin{tabular}{p{0.9cm}|p{1.7cm}|*{4}{p{0.5cm}}p{0.8cm}|*{4}{p{0.5cm}}p{0.8cm}|*{4}{p{0.5cm}}p{0.8cm}}
    \begin{tabular}{l|l|ccccc|ccccc|ccccc}
    \hline
    \textbf{Attack} & \textbf{Model} & \multicolumn{5}{c|}{\textbf{HealthcareMagic-101}} & \multicolumn{5}{c}{\textbf{Enron Email}}  & \multicolumn{5}{c}{\textbf{Synthetic Finance}} \\
    \cline{3-17}
     & & \textbf{LC} & \textbf{ULC} & \textbf{TLG} & \textbf{ASR} & \textbf{ROUGE}  & \textbf{LC} & \textbf{ULC} & \textbf{TLG} & \textbf{ASR} & \textbf{ROUGE}  & \textbf{LC} & \textbf{ULC} & \textbf{TLG} & \textbf{ASR} & \textbf{ROUGE}  \\
    \hline
    \multirow{3}{*}{TGTB} & Llama-7b-chat & 650 & 103 & 88 & 12.1 & 96.5 & 525 & 56 & 150 & 13.5 & 92.9  & 114 & 114 & 154 & 16.6 & 99.0 \\
                          & Qwen2-72B       & 701 & 130 & 42 & 6.7 & 85.2 & 550 & 112 & 127 & 11.9 & 90.2  & 250 & 250 & 149 & 20.2 & 97.0 \\
                         & ChatGPT-4    & 750 & 153 & 101  & 16.6 & 100.0 & 525   & 131 & 251 & 27.0  & 100.0  & 310   & 310 & 187 & 37.5  & 100.0  \\
    \hline
    % Repeat for PIDE, GEA, Thief, Pirate
    \multirow{3}{*}{PIDE} & Llama-7b-chat & 208 & 208 & 34 & 4.1 & 89.4 & 231 & 231 & 255 & 35.0 & 85.0 & 339 & 339 & 69 & 9.63 & 98.0 \\
                          & Qwen2-72B         & 309 & 309 & 42 & 6.8 & 94.4 & 426 & 389 & 264 & 35.2 & 92.3 & 360 & 360 & 151 & 27.0 & 99.9 \\
                         & ChatGPT-4       & 375 & 375 & 48  & 7.1 & 100.0 & 510   & 423 & 236 & 31.0  & 100.0  & 430   & 430 & 154 & 28.2  & 100.0  \\
    \hline
    \multirow{3}{*}{GEA} & Llama-7b-chat & 1,039 & 277 & 80 & 13.3 & 79.0 & 750 & 170 & 60 & 19.7 & 73.8 & 587 & 386 & 88 & 14.2 & 99.6 \\
                          & Qwen2-72B         & 1,100& 312 & 50 & 12.8 & 83.2 & 801 & 266 & 69 & 20.0 & 74.5 & 520 & 411 & 175 & 19.9 & 100.0 \\
                               & ChatGPT-4       & 1,070 & 302 & 93  & 16.0 & 100.0 & 1080   & 304 & 82 & 22.0  & 95.2  & 680   & 455 & 190 & 27.9  & 100.0  \\
    \hline
    \multirow{3}{*}{Thief} & Llama-7b-chat & 316 & 316 & 15 & 4.8 & 94.6 & 455 & 455 & 15 & 3.5 & 92.0 & 347   & 347 & 154 & 20.1  & 82.4  \\
                          & Qwen2-72B         & 330 & 330 & 13 & 3.6 & 95.7 & 535 & 535 & 27 & 3.9 & 92.4 & 403   & 403 & 197 & 23.6  & 90.4  \\
                        & ChatGPT-4       & 395 & 395 & 52  & 5.9 & 93.5 & 529   & 529 & 22 & 4.1  & 92.1  & 493   & 493 & 194 & 23.1  & 90.8 \\
    \hline
    \multirow{3}{*}{Pirate} & Llama-7b-chat & 445 & 445 & 29 & 8.8 & 90.5 & 561  &  561 & 120 & 12.0 & 90.0 & 385   & 385 & 146 & 22.1  & 93.2  \\
                          & Qwen2-72B         & 453 & 453 & 30 & 8.0 & 92.1  & 586 & 586 &  127 & 13.9 & 94.7 & 525   & 525 & 123 & 20.5  & 94.0  \\
                        & ChatGPT-4       & 486 & 486 & 75  & 13.0 & 94.4 & 609   & 609 & 324 & 30.6  & 97.6  & 520   & 520 & 420 & 31.5  & 97.2 \\
    \hline
    \multirow{3}{*}{Ours} & Llama-7b-chat & 1,099 & 574 & 349 & 62.0 & 99.4 & 1,042 & 658 & 563 & 86.4 & 99.6    & 736 & 593 & 1,081 & 99.2 & 99.9 \\
                          & Qwen2-72B      & 1,162 & 629 & 505 & 89.4 & 99.9 & 1,256 & 680 & 659 & 90.8 & 99.9 & 917 & 662 & 1,413 & 99.5 & 99.9 \\
                        & ChatGPT-4       & 1,284 & 636 & 530  & 91.9 & 100.0 & 1,492   & 711 & 735 & 93.0  & 99.5  & 1,080   & 702 & 1,011 & 99.5  & 100.0  \\
    \hline
    \end{tabular}
    }
    \caption{Targeted Attack Performance across three datasets.}
    \label{tab:target-attack-datasets}
    \vspace{-10pt}
\end{table*}



\subsection{Results of Untargeted Attack} 
We report only the \textit{leak chunks (LC)} and \textit{unique leak chunks (ULC)} as indicators of the model’s capacity to extract private information. Table~\ref{tab:untarget-attack} compares our method with five baseline approaches on the \textit{Mini-BioASQ} dataset across three LLMs. The results are consistent with those observed in the targeted attack setting.
For example, on \textit{LLaMA-7B-Chat}, our method achieves an LC of 1,782 and a ULC of 594, demonstrating strong capability in extracting diverse chunks. This effectiveness can be attributed to our use of an active learning strategy, which enhances prompt diversity and extraction performance.
Figure~\ref{fig:untarget-attack-chunks} presents similar findings on four datasets, further supporting the robustness of our approach. Representative examples of extracted private information are provided in the Appendix.



    
\begin{table}[!ht]
    \renewcommand{\arraystretch}{1.0}
    \centering
    \scriptsize % Adjust font size for single-column
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|c|c|c}
    \hline
    \textbf{Attack} & \textbf{Model} & \textbf{LC} & \textbf{ULC} & \textbf{ROUGE} \\ 
    \hline
    \multirow{3}{*}{TBTG} 
         & Llama-7b-chat & 525  & 125  & 82.3 \\
         & Qwen2-72B    & 580  & 180  & 92.4 \\
         & ChatGPT-4    & 610  & 201  & 97.0 \\
    \hline
    \multirow{3}{*}{PIDE} 
         & Llama-7b-chat & 237  & 237  & 92.0 \\
         & Qwen2-72B    & 577  & 220  & 98.5 \\
         & ChatGPT-4    & 555  & 332  & 89.2 \\
    \hline
    \multirow{3}{*}{GEA} 
         & Llama-7b-chat & 714  & 359  & 50.0 \\
         & Qwen2-72B    & 1,033 & 263  & 81.4 \\
         & ChatGPT-4    & 978  & 278  & 99.2 \\
    \hline
    \multirow{3}{*}{Thief} 
         & Llama-7b-chat & 220  & 220  & 91.7 \\
         & Qwen2-72B    & 326  & 326  & 93.9 \\
         & ChatGPT-4    & 378  & 378  & 94.5 \\
    \hline
    \multirow{3}{*}{Pirate} 
         & Llama-7b-chat & 419  & 419  & 91.7 \\
         & Qwen2-72B    & 458  & 458  & 94.0 \\
         & ChatGPT-4    & 475  & 475  & 99.2 \\
    \hline
    \multirow{3}{*}{Ours} 
         & Llama-7b-chat & 1,182 & 594  & 98.9 \\
         & Qwen2-72B    & 1,619 & 649  & 98.6 \\
         & ChatGPT-4    & 1,714 & 688  & 99.5 \\
    \hline
    \end{tabular}%
    }
    \caption{Attack performance on the HealthcareMagic-101 dataset.}
    \label{tab:untarget-attack}
    \vspace{-10pt}
\end{table}




\begin{figure}[t]
    \centering
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/attack_chunks_email.pdf}
        \caption{Eron Email.}
        \label{fig:attack-chunks-email}
    \end{subfigure}
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/attack_chunks_finance.pdf}
        \caption{Synthetic finance.}
         \label{fig:attack-chunks-finance}
    \end{subfigure}
        \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/attack_chunks_wiki.pdf}
        \caption{Mini-wikipedia.}
        \label{fig:attack-chunks-wiki}
    \end{subfigure}
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/attack_chunks_bioasq.pdf}
        \caption{Mini-BioASQ.}
        \label{fig:attack-chunks-bioasq}
    \end{subfigure}
    \caption{Comparison of extracted chunks (LC and ULC) across attacks on Llama-7b-chat and Qwen2-72B. Pale bars represent LC, and opaque bars represent ULC.}
    \label{fig:untarget-attack-chunks}
    % \vspace{-5pt}
\end{figure}



\subsection{Ablation Studies}
\label{sec:Ablation}
We conduct a series of ablation studies to investigate how key parameters affect the effectiveness of our attack in terms of privacy leakage, measured by the number of leakage chunks (LC) and unique leakage chunks (ULC).

\bheading{Returned Chunks (Top-$k$).}
To analyze the impact of the number of retrieved text chunks $k$ per query on privacy leakage, we vary $k$ among \{1, 3, 5, 7, 9\}. Experiments are conducted using the LLaMA-7B-chat model on the \texttt{HealthCareMagic} dataset, with a total of 250 untargeted attack queries. As shown in Figure~\ref{fig:ablation-topk}, the results demonstrate that increasing $k$ leads to higher values of both LC and ULC. This indicates that retrieving more chunks per query increases the likelihood and redundancy of leaked private content.

\bheading{Model Size.}
To explore the influence of model size on attack effectiveness, we evaluate five variants of LLaMA models: 7B, 8B, 13B, 33B, and 70B. Each model is tested under 250 untargeted attack queries using the same dataset. As illustrated in Figure~\ref{fig:ablation-modelsize}, larger models tend to yield higher LC and ULC values. This suggests that larger LLMs, due to their improved language understanding and generative capabilities, are more likely to extract and reproduce sensitive information during RAG responses.

\bheading{Similarity Thresholds.}
We further examine the effect of similarity thresholds used in the retrieval stage on privacy leakage. The thresholds are set to \{0.1, 0.3, 0.5, 0.7, 0.9\}, with the LLaMA-7B-chat model and the \texttt{HealthCareMagic} dataset under 250 untargeted attack attempts. Figure~\ref{fig:ablation-threshold} shows that as the similarity threshold increases, both LC and ULC tend to decrease. This is because lower similarity thresholds result in the retrieval of more loosely related or even irrelevant content, which increases the chance of retrieving sensitive data from the underlying corpus.



 
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-topk-target.pdf}
        \caption{Impact of top-$k$ selection.}
        \label{fig:ablation-topk}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-modelsize-target.pdf}
        \caption{Impact of model size.}
        \label{fig:ablation-modelsize}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-similarity-threshold-target.pdf}
        \caption{Impact of similarity threshold.}
        \label{fig:ablation-threshold}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-anchors-target.pdf}
        \caption{Impact of anchors number.}
        \label{fig:ablation-anchors}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Ablation study analyzing the impact of different parameters on extraction performance. We examine how (a) top-$k$ selection, (b) model size, (c) similarity threshold, and (d) the number of anchors  affect the number of total leak chunks (LC) and unique leak chunks (ULC).}
    \label{fig:ablation-study}
    \vspace{-5pt}
\end{figure*}


\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-topk.pdf}
        \caption{Impact of top-$k$ selection.}
        \label{fig:ablation-topk-2}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-modelsize.pdf}
        \caption{Impact of model size.}
        \label{fig:ablation-modelsize-2}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-similarity-threshold.pdf}
        \caption{Impact of similarity threshold.}
        \label{fig:ablation-threshold-2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/ablation-anchors.pdf}
        \caption{Impact of anchors number.}
        \label{fig:ablation-anchors-2}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Ablation study analyzing of untarget attacks.}
    \label{fig:ablation-study-untargeted}
    \vspace{-5pt}
\end{figure*}


% \bheading{Impact of Hyperparameters in our method: orcale test; anchor number}

\bheading{Anchors number.}
To analyze the impact of the number of anchor topics selected per iteration for generating new queries on privacy leakage, we vary the number of anchors $k$ among \{1, 3, 5, 7, 9\}. As shown in Figure~\ref{fig:ablation-anchors}, increasing the number of anchor topics leads to slightly higher values of both LC and ULC. This trend suggests that more anchor topics introduce greater query diversity, increasing the chances of covering a broader range of private content in the knowledge base and thereby enhancing the effectiveness of the attack.

\bheading{Oracle Test.}
To evaluate the effectiveness of our data estimation method in enhancing the attack success rate, we investigate the discrepancy between the estimated data distribution and the ground truth. This analysis assesses the comprehensiveness and completeness of our approach for approximating the entire underlying data distribution.
For the Oracle test, we first apply DBSCAN clustering on the ground truth dataset to obtain its distribution, denoted as $P(D)$. We then evaluate our method to derive an estimated distribution, $P'(D)$.
Subsequently, we conduct experiments on three datasets (Health, Email, and Finance) using both $P(D)$ and $P'(D)$. Table~\ref{tab:oracle-topics} presents the topics derived via the Oracle as well as those estimated from 250 queries. Figure~\ref{fig:ulc-estimation} displays the results obtained when generating 250 queries guided by $P(D)$ and $P'(D)$; while the Oracle-guided queries yield slightly higher performance in both targeted and untargeted attacks, the overall results are quite comparable.
A closer examination of the probability distributions in Figure~\ref{fig:prob-estimation}—and further corroborated by Figures~\ref{fig:health-estimation} and \ref{fig:health-estimation}—reveals substantial overlap between $P(D)$ and $P'(D)$. These results indicate that our estimation method effectively boosts attack performance, as demonstrated by the outcomes reported in Table~\ref{tab:target-attack-datasets} and Table~\ref{tab:untarget-attack}.




\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.3}
% \scriptsize
\begin{tabular}{l|c|c|c} 
    \hline
     \textbf{Model} & \textbf{Health} & \textbf{Email} & \textbf{Finance} \\ 
    \hline
 
    Oracle& xxx & xxx  & xxxx \\
   Ours   & xxx & xxx  & xxxx\\
    \hline
\end{tabular}
\caption{estimation vs oracle.}
\label{tab:oracle-topics}
\vspace{-10pt}
\end{table}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.47\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/oracle-target.pdf}
%         \caption{Target Attack.}
%         \label{fig:oracle-1}
%     \end{subfigure}
%     \vspace{4pt}
%     \begin{subfigure}{0.47\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/oracle-untarget.pdf}
%         \caption{Unargeted Attack.}
%         \label{fig:oracle-2}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{Comparison of our method and the ground truth. Pale bars represent LC, and opaque bars represent ULC.}
%     \label{fig:ulc-estimation}
%     \vspace{-5pt}
% \end{figure}




\begin{figure}[t]
    \centering
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/oracle-target.pdf}
        \caption{Targeted Attack.}
        \label{fig:oracle-1}
    \end{subfigure}
    \vspace{4pt}
    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/oracle-untarget.pdf}
        \caption{Unargeted Attack.}
        \label{fig:oracle-2}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Comparison of our method and the ground truth. Pale bars represent LC, and opaque bars represent ULC.}
    \label{fig:ulc-estimation}
    \vspace{-5pt}
\end{figure}


\begin{figure}[t]
    \centering
    % First subfigure: Health Dataset estimation
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/health-estimation.pdf}
        \caption{Health Dataset estimation.}
        \label{fig:health-estimation}
    \end{subfigure}
    \vspace{4pt}
    % Second subfigure: Unattacked or Un-targeted Attack (Email)
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/email-estimation.pdf}
        \caption{Eron Email Dataset estimation.}
        \label{fig:email-estimation}
    \end{subfigure}
    \vspace{4pt}
    % % Third subfigure: Finance Dataset estimation
    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/experiments/finance-estimation.pdf}
    %     \caption{Finance Dataset estimation.}
    %     \label{fig:finance-estimation}
    % \end{subfigure}
    % \vspace{4pt}
    \caption{Overall caption describing the experiments (e.g., Eron Email dataset estimation and related analysis).}
    \label{fig:prob-estimation}
\end{figure}



% query times: 250 300 350 400 450 500 --> it is continuous 

% FIg2:
% x: oracle  y:LC/ULC --> near the ground truth



\subsection{Overhead} 
In Table~\ref{tab:attack-time}, we report the wall-clock time (in seconds) required to prepare an attack query, send it to the RAG system, and obtain the final response. For comparison, only the results for our method and the two baselines (Pirate and Thief) are presented, because methods such as PIDE and TGTB rely on pre-designed or pre-generated queries and do not require the attack LLM to generate queries dynamically. Overall, the total execution time of our method is comparable to that of the baselines. This efficiency is achieved by selecting a small sample of anchors (even when using DBSCAN) and by employing a pre-formulated template prompt for the attacker LLM, which minimizes any computationally intensive operations within the algorithm.


\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.3}
\scriptsize
\begin{tabular}{l|c|c|c}
\hline
\textbf{Attack} & \textbf{Health} & \textbf{Email} & \textbf{Finance} \\
\hline
Thief        & $24.948{\,\pm\,}6.267$    & $24.513{\,\pm\,}4.849$    & $22.257{\,\pm\,}8.639$ \\
\hline
 Pirate        & $23.762{\,\pm\,}4.162$    & $21.909{\,\pm\,}3.786$    & $23.173{\,\pm\,}2.477$ \\
 \hline
\textbf{Ours} & $\mathbf{25.885{\,\pm\,}3.011}$ & $\mathbf{20.156{\,\pm\,}2.885}$ & $\mathbf{21.059{\,\pm\,}5.552}$ \\
\hline
\end{tabular}
\caption{Wall-clock time (seconds) to create an attack query (mean ± std)—sending it to the RAG system—getting the response.}
\label{tab:attack-time}
\end{table}




% Table 4: Wall-clock time (seconds) to create an attack query (mean ± std)–without sending it to the RAG sys- tem (Gs metric). In our attack, this includes the time to extract anchors (most cumbersome step), updated rele- vance, sample anchors, generate query. PIDE, TGTB, and GPTGEN are based on pre-designed/pre-generated queries and RThief∗ is identical to RThief (in DGEA and DGEA∗ the query creation depends on the text em- bedder which varies).
